Towards Zero-Shot Camera Trap Image Categorization

This paper describes the search for an alternative approach to the automatic categorization of camera trap images. First, we benchmark state-of-the-art classifiers using a single model for all images. Next, we evaluate methods combining MegaDetector with one or more classifiers and Segment Anything to assess their impact on reducing location-specific overfitting. Last, we propose and test two approaches using large language and foundational models, such as DINOv2, BioCLIP, BLIP, and ChatGPT, in a zero-shot scenario. Evaluation carried out on two publicly available datasets (WCT from New Zealand, CCT20 from the Southwestern US) and a private dataset (CEF from Central Europe) revealed that combining MegaDetector with two separate classifiers achieves the highest accuracy. This approach reduced the relative error of a single BEiTV2 classifier by approximately 42\% on CCT20, 48\% on CEF, and 75\% on WCT. Besides, as the background is removed, the error in terms of accuracy in new locations is reduced to half. The proposed zero-shot pipeline based on DINOv2 and FAISS achieved competitive results (1.0\% and 4.7\% smaller on CCT20, and CEF, respectively), which highlights the potential of zero-shot approaches for camera trap image categorization.

==> sections/zero-shot.tex <==
This section presents several ablations that focus on (i) benchmarking performance for CNN-based and transformer-based classifiers and (ii) testing the potential to improve the baseline performance with existing foundational models, e.g., MegaDetector (MD)~\cite{Microsoft2023MegaDetector}, Segment Anything Model (SAM)~\cite{kirillov2023segany}, DINOv2~\cite{oquab2023dinov2}, BioCLIP~\cite{stevens2024bioclip}, BLIP~\cite{li2022blip}, and ChatGPT~\cite{FreeGPT}.
